Dust temperature in ALMA $\hbox{[C $\scriptstyle\rm II $]}$-detected high-$z$ galaxies

At redshift $z>5$ the far-infrared (FIR) continuum spectra of main-sequence galaxies are sparsely sampled, often with a single data point. The dust temperature $T_{\rm d, SED}$ thus has to be assumed in the FIR continuum fitting. This introduces large uncertainties regarding the derived dust mass ($M_{\rm d}$), FIR luminosity, and obscured fraction of the star formation rate. These are crucial quantities to quantify the effect of dust obscuration in high-$z$ galaxies. To overcome observations limitations, we introduce a new method that combines dust continuum information with the overlying $\hbox{[C $\scriptstyle\rm II $]} 158\mu$m line emission. By breaking the $M_{\rm d} - T_{\rm d, SED}$ degeneracy, with our method, we can reliably constrain the dust temperature with a single observation at $158\mu$m. This method can be applied to all ALMA and NOEMA $\hbox{[C $\scriptstyle\rm II $]}$ observations and exploited in ALMA Large Programs such as ALPINE and REBELS targeting $\hbox{[C $\scriptstyle\rm II $]}$ emitters at high-$z$. We also provide a physical interpretation of the empirical relation recently found between $molecular$ gas mass and $\hbox{[C $\scriptstyle\rm II $]}$ luminosity. We derive an analogous relation linking the $total$ gas surface density and $\hbox{[C $\scriptstyle\rm II $]}$ surface brightness. By combining the two, we predict the cosmic evolution of the surface density ratio $\Sigma_{\rm H_2} / \Sigma_{\rm gas}$. We find that $\Sigma_{\rm H_2} / \Sigma_{\rm gas}$ slowly increases with redshift, which is compatible with current observations at $0 < z < 4$.

==> additional_tex_files/hyperlink_hack.tex <==

%-----------------------------------------
% avoids the 
%   \pdfendlink ended up in different nesting level than \pdfstartlink.\AtBegShi@Output ...ipout \box \AtBeginShipoutBox
% error
%-----------------------------------------
%
% see https://tex.stackexchange.com/questions/249579/pdfendlink-ended-up-in-different-nesting-level-than-pdfstartlink-error-with

% different workaround
%\AtBeginShipout{%
%  \ifnum\value{page}>1 %
%    \typeout{* Additional boxing of page `\thepage'}%
%    \setbox\AtBeginShipoutBox=\hbox{\copy\AtBeginShipoutBox}%
%  \fi
%}

\usepackage{etoolbox}
\makeatletter
\newcount\c@additionalboxlevel
\setcounter{additionalboxlevel}{0}
\newcount\c@maxboxlevel
\setcounter{maxboxlevel}{1}
\patchcmd\@combinedblfloats{\box\@outputbox}{%
  \stepcounter{additionalboxlevel}%
  \box\@outputbox
}{}{\errmessage{\noexpand\@combinedblfloats could not be patched}}

\AtBeginShipout{%
  \ifnum\value{additionalboxlevel}>\value{maxboxlevel}%
    \typeout{Warning: maxboxlevel might be too small, increase to %
      \the\value{additionalboxlevel}%
    }%
  \fi 
  \@whilenum\value{additionalboxlevel}<\value{maxboxlevel}\do{%
    \typeout{* Additional boxing of page `\thepage'}%
    \setbox\AtBeginShipoutBox=\hbox{\copy\AtBeginShipoutBox}%
    \stepcounter{additionalboxlevel}%
  }%
  \setcounter{additionalboxlevel}{0}%
}
\makeatother

